Learning Interpretable Shapelets for Time Series Classification through Adversarial Regularization

Times series classification can be successfully tackled by jointly learning a shapelet-based representation of the series in the dataset and classifying the series according to this representation. However, although the learned shapelets are discriminative, they are not always similar to pieces of a real series in the dataset. This makes it difficult to interpret the decision, i.e. difficult to analyze if there are particular behaviors in a series that triggered the decision. In this paper, we make use of a simple convolutional network to tackle the time series classification task and we introduce an adversarial regularization to constrain the model to learn more interpretable shapelets. Our classification results on all the usual time series benchmarks are comparable with the results obtained by similar state-of-the-art algorithms but our adversarially regularized method learns shapelets that are, by design, interpretable.

==> Makefile <==

# configuration variables
BASENAME=ms
pdflatex=pdflatex
image-path=images

# OPT: following line allows packages like "minted" to call external commands
#pdflatex := ${pdflatex} -shell-escape
#BIB=${BASENAME}.bib
BIB=biblioShapelets.bib


# features that are possible but not included for now (please open a feature request)
## - automatic eps to pdf
## - optimization (in terms of size) of pdf generated by inkscape, especially with embedded raster images
## - gnuplot files to svg

# (internal) tools
## recursive wildcard
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))



# (internal) derived variables
svg-files = $(call rwildcard,${image-path},*.svg)
svg-files-in-pdf = $(patsubst %.svg,%.pdf,${svg-files})
PDFDEPS = ${BASENAME}.tex $(call rwildcard,,*.bib) $(call rwildcard,,*.tex) ${svg-files-in-pdf} Makefile



# (internal) Targets of the Makefile

${BASENAME}.pdf: ${PDFDEPS}
	${pdflatex} -halt-on-error $<
	if test -f ${BIB} ; then bibtex   ${BASENAME} ; fi
	${pdflatex} $<
	${pdflatex} $<
	@echo "Making some classical checks on the pdf"
	@echo "=> looking for '?' in the PDF (that might be a missing reference)"
	@pdftotext $@ - | grep -Hrn '[?]' -  | awk '{print "   - ?: " $$0}'
	@echo "=> looking for 'TODO' in the PDF"
	@pdftotext $@ - | grep -Hrni 'TODO' -  | awk '{print "   - TODO: " $$0}'
	@echo "=> looking for 'TODO' in tex files"
	@grep -Hrni TODO $(call rwildcard,,*.tex) | awk '{print "   - TODO: " $$0}'

suppl:
	make BASENAME=aistats_2018_supplementary_format

fast:
	make ${PDFDEPS}
#	${BASENAME}.tex $(call rwildcard,,*.bib) $(call rwildcard,,*.tex)
	if test -f ${BASENAME}.bib ; then bibtex ${BASENAME} || make ; fi
	${pdflatex} -halt-on-error ${BASENAME}.tex

continuous:
	make fast
	(which inotifywait && inotifywait -r -m . --exclude '^[.]#.*|#.*|.*~|${BASENAME}[.][^t]..$$' -e MODIFY -e CREATE | while read line ; do echo =================== $$line; make fast ; done) || true
	which inotifywait || while true ; do sleep .25; for i in ${PDFDEPS} ; do if test $$i -nt ${BASENAME}.pdf ; then make fast; break; fi ; done ; done

.PHONY: export export-images clean latexdiff fast continuous

clean:
	rm -f ${BASENAME}.pdf ${BASENAME}.aux ${BASENAME}.bbl ${BASENAME}.blg ${BASENAME}.log ${BASENAME}.toc

$(svg-files-in-pdf): %.pdf: %.svg
	inkscape -T $(patsubst %.pdf,%.svg,$@) --export-pdf=$@

reconvert-svg:
	make $(svg-files-in-pdf)

export:
	rm -rf export
	mkdir export
	cat ${BASENAME}.tex | awk '/\\listfiles/ {next} /\\documentclass.*/ {print; print "\\listfiles"; next} // {print}' > ,,.tex
	cp ${BASENAME}.tex export/
# adding the base tex file (as it is not listed)
# adding the bibs also (as it uses the bbl actually) as they are useful to rebuild from scratch
	for i in ${BASENAME}.tex $$(find . -name \*.bib) $$(${pdflatex} ,,.tex | awk '/ *\*File List\*/ {show=1; next;} / \*\*\*\*\*+/ {show=0;next} // {if (show) {print}}') ; do if test -f $$i ; then mkdir -p export/$$(dirname $$i) && cp $$i export/$$(dirname $$i)/ ; fi ; done
	rm -f ,,.tex
	echo > export/Makefile
	echo ${BASENAME}.pdf: >> export/Makefile
	echo "	"${pdflatex} ${BASENAME}.tex >> export/Makefile
	if test -f ${BIB} ; then echo "	"bibtex ${BASENAME} >> export/Makefile ; fi
	echo "	"${pdflatex} ${BASENAME}.tex >> export/Makefile
	echo "	"${pdflatex} ${BASENAME}.tex >> export/Makefile
	echo .PHONY: ${BASENAME}.pdf >> export/Makefile


# used to export images (for IEEE journal(s?)): might need to adapt things (especially if you have tables to skip), need to uncomment update the choice of the teaser image and the author names.
export-images:
	make reconvert-svg
	rm -rf export-images
	mkdir export-images
	cat ${BASENAME}.tex | awk ' /\\begin{document}.*/ {print "\\usepackage[active,floats,graphics,tightpage,pdflatex]{preview}" ; print "\\renewcommand{\\caption}[1]{}" ; print ; next} // {print}' > ,,.tex
	${pdflatex} ,,.tex
	if test -f ${BIB} ; then bibtex   ,, ; fi
	${pdflatex} ,,.tex
	${pdflatex} ,,.tex
##	 extract and convert each page, pdftk not working here... but don't know why
	for i in $$(seq 30)  ; do pdftops -eps -level3 -f $$i -l $$i ,,.pdf export-images/"Figure $$i.eps" || true           ; done
##	if you have to skip things (e.g., due to a table), change the seq above and use the below to complete (it offsets by one with the "-1")… take inspiration
#	for i in 21 22 23 24 25 26 27 28 ; do pdftops -eps -level3 -f $$i -l $$i ,,.pdf export-images/"Figure $$(($$i - 1)).eps" ; done
## 	Below: use special raster option to convert an image with anoying semi transparent things
#	pdftops -eps -level3 -f 28 -l 28 -r 1800 ,,.pdf export-images/"Figure 27.eps"
##	Below: other files
#	cp export-images/"Figure 1.eps" export-images/"Teaser Image.eps"
#	cp images/guy1.jpg export-images/
#	cp images/guy2.jpg export-images/
#	cp images/guy3.jpg export-images/
#	cp Author-Copies-tpami.pdf export-images/
	rm -f ,,.tex



with=NONE
latexdiff:
	@test ${with} '!=' NONE || (echo -n "\n\nPlease check you saved/commited everything and use something like \n    make latexdiff with=HEAD^\n\n"; false)
	rm -rf ,,latexdiff
	mkdir ,,latexdiff
	git rev-parse --abbrev-ref HEAD  | sed 's@^refs/heads/@@g' > ,,latexdiff.br
	test $$(cat ,,latexdiff.br) '!=' "HEAD"
	git stash save "Before latexdiff"
	git checkout ${with}
	for i in $$(find . -name \*.tex) ; do mkdir -p ,,latexdiff/$$(dirname $$i) && cp $$i ,,latexdiff/$$(dirname $$i)/ ; done
	cat ,,latexdiff.br | xargs git checkout
	rm -f ,,latexdiff.br
	latexdiff ,,latexdiff/${BASENAME}.tex ${BASENAME}.tex > diff && mv diff ${BASENAME}.tex
	make BASENAME=${BASENAME} || (echo -n "\n\nCompilation of diff'ed latex failed.\nPlease fix it, make and do whatever you want with the pdf.\nTHEN, run:\n    git reset --hard ; git stash apply\n\n" ; false) 
	mv ${BASENAME}.pdf latexdiff.pdf
	rm -rf ,,latexdiff
	@echo ""
	@echo "INFO: Your diff file is in latexdiff.pdf"
	@echo ""
	@echo "now reseting"
	git reset --hard
	@echo "INFO: If you had uncommited changes, they have been stashed."
	@echo "      Please check and reapply them only if needed (git stash apply)"
#	git stash apply || echo "INFO: stash apply might fail if nothing was uncommited"


